SHATTER: Control and Defense-Aware Attack Analytics for Activity-Driven Smart Home Systems

Modern smart home control systems utilize real-time occupancy and activity monitoring to ensure control efficiency, occupants' comfort, and optimal energy consumption. Moreover, adopting machine learning-based anomaly detection models (ADMs) enhances security and reliability. However, sufficient system knowledge allows adversaries/attackers to alter sensor measurements through stealthy false data injection (FDI) attacks. Although ADMs limit attack scopes, the availability of information like occupants' location, conducted activities, and alteration capability of smart appliances increase the attack surface. Therefore, performing an attack space analysis of modern home control systems is crucial to design robust defense solutions. However, state-of-the-art analyzers do not consider contemporary control and defense solutions and generate trivial attack vectors. To address this, we propose a control and defense-aware novel attack analysis framework for a modern smart home control system, efficiently extracting ADM rules. We verify and validate our framework using a state-of-the-art dataset and a prototype testbed.

==> sections/Findings-Discussion-and-Future-Direction.tex <==
%
\section{Findings and Discussion}
\label{sec:findings}
%
%\nur{In our research, we have identified a tool for }

Our research has identified many challenges that opened a broad domain of future research scope. 
\begin{itemize}
    \item \revise{Scalability analysis has shown the infeasibility of exploring the whole search space in a feasible amount of time with sufficiently high computation power. Optimization of attack vectors (i.e., attack routine) through a meta-heuristic algorithm can be considered in future works.}
    \item \revise{Although some modern smart homes generate their own energy to meet their energy demands and store any excess energy in an energy storage system like a battery, our current modeling does not account for this renewable energy. If there is excess energy production, the home can be viewed as a microgrid and sell the excess energy to the grid. Even though SHATTER-identified attacks will unquestionably decrease earnings compared to a benign operating condition, the attack's impact in this scenario will be distinct and needs attention. In our future attack modeling, we will factor in renewable power sources.}
\end{itemize}


\begin{table}[]
\caption{Primary differences in between BIoTA and SHATTER framework.}
\label{tab:biota_vs_shatter}
\revise{
\begin{tabular}{|p{2.3cm}|p{2.7cm}|p{2.7cm}|}
\hline
\textbf{Criteria}                                                               & \textbf{BIoTA}                                                                                                      & \textbf{SHATTER}                                                                                                                      \\ \hline
\textbf{Application Domain}                                                     & Smart building/ homes                                                                                               & Smart homes                                                                                                                           \\ \hline
\textbf{Number of Occupants}                                                    & $\sim$(10-1000)                                                                                                     & $\sim$(1-10)                                                                                                                          \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Anomaly Detection\\ Model\end{tabular}}      & Rule-based                                                                                                          & Machine Learning-based                                                                                                                \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Occupant's Activity\\ Tracking\end{tabular}} & Not considered                                                                                                      & Considered                                                                                                                         \\ \hline
\textbf{Appliance Modeling}                                                     & Considers fixed load at every control cycle                               & Takes appliance load (including IoT device triggering) into consideration for modeling 
\\ \hline
\textbf{Attack Constraints}                                                     & Stealthy FDI attack to bypass control system                              & Stealthy FDI attack to bypass both control system and occupants                             \\ \hline
\textbf{Attack Goal}                                                            & Increment in energy consumption or occupants\'s discomfort & Both increment in energy consumption and occupant's discomfort                              \\ \hline
\textbf{Attack Technique}                                                            & Greedy FDI attack to manipulate both IAQ and appliance sensor measurements & Dynamic FDI to stealthily manipulate both IAQ and appliance sensor measurements                              \\ \hline
\end{tabular}}
\end{table}



==> tex-figures/Tex-Figure_ADM_House-A.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%% ASHRAE vs SHATTER Control Cost %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
%\vspace{-6pt}
    \begin{center}
         \subfigure[]
        {
        \label{subfig:anomaly_detection_acuracy_house_A_occ_1}
            \includegraphics[width=0.46\columnwidth]{plots/ADM-House_A_Occ-1.pdf}
        }
        \subfigure[]
        {
        \label{subfig:anomaly_detection_acuracy_house_A_occ_2}
            \includegraphics[width=0.46\columnwidth]{plots/ADM-House_A_Occ-2.pdf}
        }     
    \end{center}
    \vspace{-12pt}
    \caption{Progressive Anomaly Detection Accuracy for (a) ARAS Occupant: O-1 (b) ARAS Occupant: O-2 of House-A.}
    \label{fig:anomaly_detection_acuracy}
    \vspace{-12pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex-figures/Tex-Figure_ASHRAE-vs-SHATTER_Control-Cost.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%% ASHRAE vs SHATTER Control Cost %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\vspace{-6pt}
    \begin{center}
         \subfigure[]
        {
        \label{subfig:control_cost_comparison_house_A}
            \includegraphics[width=0.48\columnwidth]{plots/House-A_ASHRAE-vs-SHATTER-Control-Cost.pdf}
        }\hspace{-9pt}
        \subfigure[]
        {
        \label{subfig:control_cost_comparison_house_B}
            \includegraphics[width=0.48\columnwidth]{plots/House-B_ASHRAE-vs-SHATTER-Control-Cost.pdf}
        }     
    \end{center}
    \vspace{-12pt}
    \caption{Comparison between ASHRAE and proposed Control Cost (\$) for (a) ARAS House-A (b) ARAS House-B.}
    \label{fig:control_cost_comparison}
    \vspace{-17pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex-figures/Tex-Figure_BIoTA-vs-SHATTER-Attack.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%% ASHRAE vs SHATTER Control Cost %%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% ASHRAE vs SHATTER Control Cost %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
%\vspace{-6pt}
    \begin{center}
         \subfigure[]
        {\label{subfig:attack_cost_comparison_house_A}
            \includegraphics[width=0.45\columnwidth]{plots/House-A_BIoTA-vs-SHATTER-Attack-Cost.pdf}
        }
        \subfigure[]
        {\label{subfig:attack_cost_comparison_house_B}
            \includegraphics[width=0.45\columnwidth]{plots/House-B_BIoTA-vs-SHATTER-Attack-Cost.pdf}
        }     
    \end{center}
    \vspace{-12pt}
    \caption{Comparison in between SHATTER Attack Impact with BIoTA.}
    \vspace{-9pt}
    \label{fig:control_cost_comparison}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex-figures/Tex-Figure_Cluster_House-A.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%% ASHRAE vs SHATTER Control Cost %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!tb]
\centering
\includegraphics[width = 0.33\textwidth]{plots/Clusters-House_A_Occ-1.pdf}
\centering
\vspace{-10pt}
\caption{Cluster Visualizations of ADM for ARAS House A (Occupant O-1).}
\label{fig:cluster_house_A_occ_1}
\vspace{-15pt}
\end{figure}

% \begin{figure}[!t]
% %\vspace{-6pt}
%     \begin{center}
%          \subfigure[]
%         {
%         \label{subfig:cluster_house_A_occ_1}
%             \includegraphics[width=0.90\columnwidth]{plots/Clusters-House_A_Occ-1.pdf}
%         }
%         % \subfigure[]
%         % {
%         % \label{subfig:cluster_house_A_occ_2}
%         %     \includegraphics[width=0.90\columnwidth]{plots/Clusters-House_A_Occ-2.pdf}
%         % }     
%     \end{center}
%     \vspace{-12pt}
%     \caption{Cluster Visualizations of ADM for (a) ARAS Occupant: O-1 (b) ARAS Occupant: O-2 of House-A.}
%     \label{fig:cluster}
%     \vspace{-9pt}
% \end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex-figures/Tex-Figure_Proposed-Attack-Scenario.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width = 0.45\textwidth]{figures/Testbed-Plan_Attack-2.pdf}
\centering
\vspace{-9pt}
\caption{Prototype testbed architecture.}
\label{fig:attack_scenarios}
\vspace{-15pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex-figures/Tex-Figure_Proposed-Attack-Technique.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width = 0.48\textwidth]{figures/MitM-ARP-Using-Ettercap.pdf}
\centering
%\vspace{1pt}
\caption{Proposed Attack Technique}
\label{fig:attack_technique}
\vspace{-15pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex-figures/Tex-Figure_Testbed.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%% Scalability Real Figure %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
\vspace{-3pt}
    \begin{center}
        \subfigure[]
        {
        \label{subfig:testbed}
            \includegraphics[width=0.51\columnwidth]{figures/Testbed.png}
        }
        %\hspace{6pt}
        \subfigure[]
        {
        \label{subfig:control}
            \includegraphics[width=0.42\columnwidth]{figures/Control.pdf}
        }
        %\hspace{6pt}     
        % \subfigure[]
        % {
        % \label{subfig:attack}
        %     \includegraphics[width=0.59\columnwidth]{figures/Attack.png}
        % }
        %\hspace{6pt}
\end{center}
\vspace{-15pt}
\caption{(a) Demonstrates a testbed instance, when Alice is showering in the bathroom zone, and Bob is taking nap in the Bedroom zone, where (b) shows the benign control scenario, where bathroom and bedroom zone vents are open and is getting air supply to neutralize the added heat generated from the two occupants, corresponding zone lights and the smart bathtub appliance.}
\label{fig:testbed}
\vspace{-9pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex-figures/Text-Figure_Components_Control-System.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width = 0.35\textwidth]{figures/Components_Control-System.pdf}
\centering
\vspace{-9pt}
\caption{Smart Home HVAC Control System with HVAC Controller.}
\label{fig:system-components}
\vspace{-6pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex-figures/Text-Figure_Overview_Control-System.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width = 0.96\columnwidth]{figures/Overview_Control-System.pdf}
\vspace{-9pt}
\caption{Smart Home System with HVAC Controller.}
\label{fig:system-overview}
\vspace{-12pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex-figures/Text-Figure_Scalability.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%% Scalability %%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[!t]
%\vspace{-6pt}
    \begin{center}
         \subfigure[]
        {
        \label{subfig:scalability_time_horizon}
            \includegraphics[width=0.48\columnwidth]{plots/Scalability_Time_Horizon.pdf}
        }
        \hspace{-8pt}
        \subfigure[]
        {
        \label{subfig:scalability_horizontal}
            \includegraphics[width=0.46\columnwidth]{plots/Scalability_Horizontal.pdf}
        }     
    \end{center}
    \vspace{-12pt}
    \caption{Scalability analysis based on (a) time horizon, (b) horizontal scaling.}
    \label{fig:scalability}
    \vspace{-15pt}
\end{figure}
%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> tex-tables/Tex-Table_Activity-Appliances-Map.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\scriptsize
\centering
\caption{Smart Home Control System Modeling Parameters Demonstrating the Activity-Based Energy Consumption of Occupants/ Appliances and Mapping between Various Occupant Activities and Appliances Status (0: OFF, 1: ON)}
\label{tab:activity-appliances-map}
\begin{tabular}{|l|l|l|lllllllllllll|l|l|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Activity\\ ID\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Activity}}}        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Zone \\ ID\end{tabular}}}} & \multicolumn{13}{c|}{\textbf{Appliances Status (On/Off) in Benign Scenario}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}PP $CO_2$ \\(CFM)\end{tabular}}}} & \multicolumn{1}{c|}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}PP Heat \\(W)\end{tabular}}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}l@{}}Total\\ Cost\\ (W)\end{tabular}}} \\ \cline{4-16}
\multicolumn{1}{|c|}{}                                                                                & \multicolumn{1}{c|}{}                                          & \multicolumn{1}{c|}{}                                                                             & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}BL\\ (1)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}LL\\ (2)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}KL \\ (3)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}BL\\ (4)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}ST\\ (3)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}O\\ (3)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}M\\ (3)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}BT \\ (4)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}W\\ (3)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}D\\ (3)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}DW\\ (3)\end{tabular}}} & \multicolumn{1}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}MC\\ (1)\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}l@{}}SF\\ (2)\end{tabular}} & \multicolumn{1}{c|}{}                                                                                                & \multicolumn{1}{c|}{}                                                                                               &                                                                                      \\ \hline
A-1                                                                                                   & Other                                                          & Z-0                                                                                     & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0                                                                                                                    & 0                                                                                                                   & 0                                                                                    \\ \hline
A-2                                                                                                   & Going Out                                                      & Z-0                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0                                                                                                                    & 0                                                                                                                   & 0                                                                                    \\ \hline
A-3                                                                                                   & \begin{tabular}[c]{@{}l@{}}Preparing \\ Breakfast\end{tabular} & Z-3                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{1}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1335                                                                                                               & 133.49                                                                                                              & 5127                                                                                 \\ \hline
A-4                                                                                                   & \begin{tabular}[c]{@{}l@{}}Having \\ Breakfast\end{tabular}    & Z-3                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{1}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1132                                                                                                               & 113.26                                                                                                              & 52                                                                                   \\ \hline
A-5                                                                                                   & \begin{tabular}[c]{@{}l@{}}Preparing \\ Lunch\end{tabular}     & Z-3                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{1}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1335                                                                                                               & 133.49                                                                                                              & 5127                                                                                 \\ \hline
A-6                                                                                                   & \begin{tabular}[c]{@{}l@{}}Having \\ Lunch\end{tabular}        & Z-3                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1132                                                                                                               & 113.26                                                                                                              & 27                                                                                   \\ \hline
A-7                                                                                                   & \begin{tabular}[c]{@{}l@{}}Preparing \\ Dinner\end{tabular}    & Z-3                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{1}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1335                                                                                                               & 133.49                                                                                                              & 5127                                                                                 \\ \hline
A-8                                                                                                   & \begin{tabular}[c]{@{}l@{}}Having \\ Dinner\end{tabular}       & Z-3                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{1}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1132                                                                                                               & 113.26                                                                                                              & 52                                                                                   \\ \hline
A-9                                                                                                   & \begin{tabular}[c]{@{}l@{}}Washing \\ Dishes\end{tabular}      & Z-3                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1213                                                                                                               & 121.35                                                                                                              & 1827                                                                                 \\ \hline
A-10                                                                                                  & \begin{tabular}[c]{@{}l@{}}Having \\ Snack\end{tabular}        & Z-3                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{1}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1132                                                                                                               & 113.26                                                                                                              & 52                                                                                   \\ \hline
A-11                                                                                                  & Sleeping                                                       & Z-1                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.0384                                                                                                               & 38.43                                                                                                               & 0                                                                                    \\ \hline
A-12                                                                                                  & \begin{tabular}[c]{@{}l@{}}Watching \\ TV\end{tabular}         & Z-2                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 1                                                         & 0.0607                                                                                                               & 60.67                                                                                                               & 245                                                                                  \\ \hline
A-13                                                                                                  & Studying                                                       & Z-2                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 1                                                         & 0.0525                                                                                                               & 52.58                                                                                                               & 245                                                                                  \\ \hline
A-14                                                                                                  & \begin{tabular}[c]{@{}l@{}}Having \\ Shower\end{tabular}       & Z-4                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{1}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1011                                                                                                               & 101.13                                                                                                              & 1518                                                                                 \\ \hline
A-15                                                                                                  & Toileting                                                      & Z-4                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1496                                                                                                               & 149.67                                                                                                              & 18                                                                                   \\ \hline
A-16                                                                                                  & Napping                                                        & Z-1                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.0384                                                                                                               & 38.43                                                                                                               & 0                                                                                    \\ \hline
A-17                                                                                                  & \begin{tabular}[c]{@{}l@{}}Using \\ Internet\end{tabular}      & Z-1                                                                                               & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                         & 0                                                         & 0.0606                                                                                                               & 60.67                                                                                                               & 256                                                                                  \\ \hline
A-18                                                                                                  & \begin{tabular}[c]{@{}l@{}}Reading \\ Book\end{tabular}        & Z-2                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 1                                                         & 0.0607                                                                                                               & 60.67                                                                                                               & 245                                                                                  \\ \hline
A-19                                                                                                  & Laundry                                                        & Z-3                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{1}                                                        & \multicolumn{1}{l|}{1}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1132                                                                                                               & 113.26                                                                                                              & 3127                                                                                 \\ \hline
A-20                                                                                                  & Shaving                                                        & Z-4                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.0809                                                                                                               & 80.90                                                                                                               & 18                                                                                   \\ \hline
A-21                                                                                                  & \begin{tabular}[c]{@{}l@{}}Brushing \\ Teeth\end{tabular}      & Z-4                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.0809                                                                                                               & 80.90                                                                                                               & 18                                                                                   \\ \hline
A-22                                                                                                  & \begin{tabular}[c]{@{}l@{}}Talking on \\ Phone\end{tabular}    & Z-2                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 1                                                         & 0.0606                                                                                                               & 60.67                                                                                                               & 245                                                                                  \\ \hline
A-23                                                                                                  & \begin{tabular}[c]{@{}l@{}}Listening to \\ Music\end{tabular}  & Z-1                                                                                               & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1618                                                                                                               & 161.81                                                                                                              & 36                                                                                   \\ \hline
A-24                                                                                                  & Cleaning                                                       & Z-3                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.1537                                                                                                               & 153.72                                                                                                              & 27                                                                                   \\ \hline
A-25                                                                                                  & \begin{tabular}[c]{@{}l@{}}Having \\ Conversation\end{tabular} & Z-2                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{1}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 1                                                         & 0.0728                                                                                                               & 72.81                                                                                                               & 270                                                                                  \\ \hline
A-26                                                                                                  & \begin{tabular}[c]{@{}l@{}}Having \\ Guest\end{tabular}        & Z-2                                                                                               & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{1}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 1                                                         & 0.0606                                                                                                               & 60.67                                                                                                               & 270                                                                                  \\ \hline
A-27                                                                                                  & \begin{tabular}[c]{@{}l@{}}Changing \\ Clothes\end{tabular}    & Z-1                                                                                               & \multicolumn{1}{l|}{1}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                          & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                        & \multicolumn{1}{l|}{0}                                                         & \multicolumn{1}{l|}{0}                                                         & 0                                                         & 0.0889                                                                                                               & 88.99                                                                                                               & 36                                                                                   \\ \hline
\end{tabular}
\end{table*}

==> tex-tables/Tex-Table_Appliances-Attack_Appliances.tex <==
\begin{table}[t]
\small
\centering
\caption{Appliance Triggering Attack Impact with Various Appliance Triggering Capability}
\label{tab:ams_contribution_appliance}
\vspace{-6pt}
\scriptsize
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Number of } \\ \textbf{Accessible Appliances}\end{tabular}}                                  & \begin{tabular}[c]{@{}l@{}}\textbf{House A} \\ \textbf{Energy Cost (\$)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{House B} \\ \textbf{Energy Cost (\$)}\end{tabular} \\ \hline
13 Appliances                                                               & 48.09           & 28.21          \\ \hline
\begin{tabular}[c]{@{}l@{}}8 Appliances\end{tabular}  & 43.33           & 24.25        \\ \hline
\begin{tabular}[c]{@{}l@{}}3 Appliances\end{tabular} & 37.37           & 22.083          \\ \hline
\end{tabular}
\vspace{-9pt}
\end{table}

==> tex-tables/Tex-Table_Appliances-Attack_Zones.tex <==
\begin{table}[]
\small
\centering
\caption{Appliance Triggering Attack Impact with Various Zone Measurement Access Capability}
\vspace{-6pt}
\scriptsize
\label{tab:ams_contribution_zones}
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}\textbf{Number of } \\ \textbf{Accessible Zone}\end{tabular}}                                  & \begin{tabular}[c]{@{}l@{}}\textbf{House A} \\ \textbf{Energy Cost (\$)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{House B} \\ \textbf{Energy Cost (\$)}\end{tabular} \\ \hline
4 Zones                                                               & 124.93           & 60.03          \\ \hline
\begin{tabular}[c]{@{}l@{}}3 Zones\end{tabular}  & 43.33           & 15.27          \\ \hline
\begin{tabular}[c]{@{}l@{}}2 Zones\end{tabular} & 13.03           & 2.11           \\ \hline
\end{tabular}
\vspace{-9pt}
\end{table}

==> tex-tables/Tex-Table_Appliances-Information.tex <==
\begin{table}[]
\small
\centering
\caption{Smart Home Control System Modeling Parameters Demonstrating the Location and Energy Consumption of Various Appliances}
\label{tab:Applaiances-Information}
\begin{tabular}{|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Appliance \\ ID\end{tabular}}} & \multicolumn{1}{c|}{\textbf{Appliance}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Zone \\ ID\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Energy \\ (W)\end{tabular}}} \\ \hline
App-1                                                                                  & Bedroom Light (BL)                      & Z-1                                   & 36                                                                                 \\ \hline
App-2                                                                                  & Livingroom Light (LL)                   & Z-2                                   & 45                                                                                 \\ \hline
App-3                                                                                  & Kitchen Light (KL)                      & Z-3                                   & 27                                                                                 \\ \hline
App-4                                                                                  & Bathroom Light (BTL)                    & Z-4                                   & 18                                                                                 \\ \hline
App-5                                                                                  & Stove (ST)                              & Z-3                                   & 2100                                                                               \\ \hline
App-6                                                                                  & Oven (O)                                & Z-3                                   & 3000                                                                               \\ \hline
App-7                                                                                  & Mug (M)                                 & Z-3                                   & 25                                                                                 \\ \hline
App-8                                                                                  & Bathtub (BT)                            & Z-4                                   & 1500                                                                               \\ \hline
App-9                                                                                  & Washer (W)                              & Z-3                                   & 1000                                                                               \\ \hline
App-10                                                                                 & Dryer (D)                               & Z-3                                   & 2100                                                                               \\ \hline
App-11                                                                                 & Dishwasher (DW)                         & Z-3                                   & 1800                                                                               \\ \hline
App-12                                                                                 & Massage Chair (MC)                      & Z-1                                   & 220                                                                                \\ \hline
App-13                                                                                 & Smart Sofa                              & Z-2                                   & 200                                                                                \\ \hline
\end{tabular}
\end{table}

==> tex-tables/Tex-Table_Case-Studies.tex <==
\begin{table*}[!t]
\centering
\scriptsize
\caption{Case study}
\vspace{-6pt}
\label{tab:case-studies}
\begin{tabular}{|l|l|cl|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Schedule}}        & \multirow{2}{*}{\textbf{Occupant}} & \multicolumn{1}{l|}{\textbf{Time}}     & \textbf{6:00 PM} & \textbf{6:01 PM} & \textbf{6:02 PM} & \textbf{6:03 PM} & \textbf{6:04 PM} & \textbf{6:05 PM} & \textbf{6:06 PM} & \textbf{6:07 PM} & \textbf{6:08 PM} & \textbf{6:09 PM} \\ \cline{3-13} 
                                          &                                    & \multicolumn{1}{l|}{\textbf{Slot (t)}} & \textbf{1080}    & \textbf{1081}    & \textbf{1082}    & \textbf{1083}    & \textbf{1084}    & \textbf{1085}    & \textbf{1086}    & \textbf{1087}    & \textbf{1088}    & \textbf{1089}    \\ \hline
\multirow{2}{*}{\textbf{Actual}}          & \textbf{Alice}                     & \multicolumn{2}{c|}{2}                                    & 2                & 2                & 2                & 2                & 2                & 2                & 2                & 2                & 2                \\ \cline{2-13} 
                                          & \textbf{Bob}                       & \multicolumn{2}{c|}{0}                                    & 0                & 0                & 0                & 0                & 0                & 0                & 0                & 0                & 0                \\ \hline
\multirow{2}{*}{\textbf{Greedy}}          & \textbf{Alice}                     & \multicolumn{2}{c|}{2}                                    & 2                & 2                & 2                & 2                & 2                & 2                & 2                & 2                & 2                \\ \cline{2-13} 
                                          & \textbf{Bob}                       & \multicolumn{2}{c|}{0}                                    & 0                & 0                & 0                & 0                & 0                & 0                & 0                & 0                & 0                \\ \hline
\multirow{2}{*}{\textbf{SHATTER}}         & \textbf{Alice}                     & \multicolumn{2}{c|}{2}                                    & 2                & 2                & 2                & 2                & 2                & 3                & 3                & 4                & 4                \\ \cline{2-13} 
                                          & \textbf{Bob}                       & \multicolumn{2}{c|}{2}                                    & 2                & 2                & 2                & 2                & 2                & 2                & 2                & 2                & 2                \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Range} \\ \textbf{Threshold}\end{tabular}} & \textbf{Alice}                     & \multicolumn{2}{c|}{{[}9 - 30{]}}                         & {[}10 - 27{]}    & {[}10 - 25{]}    & {[}10 - 22{]}    & {[}11 - 16{]}    & {[}11 - 19{]}    & {[}11 - 13{]}    & {[}{]}           & {[}75 - 75{]}    & {[}66 - 75{]}    \\ \cline{2-13} 
                                          & \textbf{Bob}                       & \multicolumn{2}{c|}{{[}5-11{]}}                           & {[}9-18{]}       & {[}5-11{]}       & {[}9-18{]}       & {[}16-19{]}      & {[}9-18{]}       & {[}25-31{]}      & {[}8-18{]}       & {[}9-18{]}       & {[}1-9{]}        \\ \hline
\multirow{2}{*}{\textbf{Trigger Status}}  & \textbf{Alice}                     & \multicolumn{2}{c|}{False}                                & False            & False            & False            & False            & False            & True             & True             & True             & False            \\ \cline{2-13} 
                                          & \textbf{Bob}                       & \multicolumn{2}{c|}{True}                                 & True             & True             & True             & True             & False            & False            & False            & False            & False            \\ \hline
\end{tabular}
\vspace{-9pt}
\end{table*}

==> tex-tables/Tex-Table_Zone-Information.tex <==
\begin{table}[]
\small
\centering
\caption{Smart Home Control System Modeling Parameters Demonstrating the ASHRAE-Based Zone Information.}
\label{tab:Zone-Information}
\begin{tabular}{|c|l|l|l|l|l|}
\hline
\textbf{Zone ID} & \multicolumn{1}{c|}{\textbf{Zone}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}PP \\$CO_2$ \\ (CFM)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}PP \\ Heat \\(W)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}App \\ Heat \\(W)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Vol \\ (CF)\end{tabular}}} \\ \hline
Z-0              & Outdoor                            & 0                                                                                                               & 0                                                                                                                 & 0                                                                                                                  & 1                                                                                    \\ \hline
Z-1              & Bedroom                            & 0.019                                                                                                           & 93.005                                                                                                            & 136                                                                                                                & 2592                                                                                 \\ \hline
Z-2              & Livingroom                         & 0.013                                                                                                           & 63.635                                                                                                            & 245                                                                                                                & 2880                                                                                 \\ \hline
Z-3              & Kitchen                            & 0.0272                                                                                                          & 133.144                                                                                                           & 3000                                                                                                               & 2304                                                                                 \\ \hline
Z-4              & Bathroom                           & 0.0221                                                                                                          & 108.1795                                                                                                          & 1500                                                                                                               & 1728                                                                                 \\ \hline
\end{tabular}
\end{table}
